Task-Oriented Paraphrase Analytics

Since paraphrasing is an ill-defined task, the term "paraphrasing" covers text transformation tasks with different characteristics. Consequently, existing paraphrasing studies have applied quite different (explicit and implicit) criteria as to when a pair of texts is to be considered a paraphrase, all of which amount to postulating a certain level of semantic or lexical similarity. In this paper, we conduct a literature review and propose a taxonomy to organize the 25~identified paraphrasing (sub-)tasks. Using classifiers trained to identify the tasks that a given paraphrasing instance fits, we find that the distributions of task-specific instances in the known paraphrase corpora vary substantially. This means that the use of these corpora, without the respective paraphrase conditions being clearly defined (which is the normal case), must lead to incomparable and misleading results.

==> fig-paraphrase-task-taxonomy-equiv.tex <==
\tikzset{
  basic/.style  = {draw, rectangle, minimum height=2em},
  root/.style   = {basic, thin, align=center, draw=none},
  level 1/.style = {basic, thin, align=center, sibling distance=24em, level distance=4em},
  level 2/.style = {basic, thin, align=center, sibling distance=12.5em},
  level 3/.style = {basic, thin, align=center, text width=8em},
  level 4/.style = {basic, thin, align=left, text width=10em}
}


\bgroup
\small
\centering
\begin{tikzpicture}[
edge from parent/.style={<-,draw},
>=latex]

% root of the the initial tree, level 1
\node[root] {\bf Paraphrase generation task}
% The first level, as children of the initial tree
child {node[level 2] (c1) {Semantically equivalent paraphrasing}
child {node[level 3] (c11) {Copy editing}}
child {node[level 3] (c12) {Data augmentation}}
child {node[level 3] (c13) {Linguistic steganography}}
child {node[level 3] (c14) {Style adjustment}}};

\begin{scope}[every node/.style={level 4}]
%\node [below of = c11, xshift=2em] (c111) {Document layout optimization};
\node [below of = c11, xshift=2em] (c112) {Improvement of coherence};
\node [below of = c112] (c113) {Text simplification};
\node [below of = c113] (c114) {Sentence compression / expansion};

\node [below of = c12, xshift=2em] (c121) {Adversarial example generation};

\node [below of = c13, xshift=2em] (c131) {Acrostification};
\node [below of = c131] (c132) {Natural language watermarking};

\node [below of = c14, xshift=2em] (c141) {Author obfuscation};
\node [below of = c141] (c142) {Plagiarizing};
\node [below of = c142] (c143) {Style transfer};
\end{scope}

% lines from each level 3 node to every one of its children
\foreach \value in {2,3,4}
\draw[<-] (c11.south west) |- (c11\value.west);

\foreach \value in {1}
\draw[<-] (c12.south west) |- (c12\value.west);

\foreach \value in {1,2}
\draw[<-] (c13.south west) |- (c13\value.west);

\foreach \value in {1,2, 3}
\draw[<-] (c14.south west) |- (c14\value.west);

\end{tikzpicture}
\egroup




==> fig-paraphrase-task-taxonomy-sim.tex <==
\tikzset{
  basic/.style  = {draw, rectangle, minimum height=2em},
  root/.style   = {basic, thin, align=center, draw=none, level distance=0em},
  level 1/.style = {basic, thin, align=center, sibling distance=24em, level distance=4em},
  level 2/.style = {basic, thin, align=center, sibling distance=10.5em},
  level 3/.style = {basic, thin, align=center, text width=6em},
  level 4/.style = {basic, thin, align=left, text width=8em}
}



\bgroup
\small
\centering
\begin{tikzpicture}[
edge from parent/.style={<-,draw},
>=latex]

% root of the the initial tree, level 1
\node[root] {\bf Paraphrase generation task}
% The first level, as children of the initial tree
child {node[level 2] (c2) {Semantically similar paraphrasing}
child {node[level 3] (c21) {Context change}}
child {node[level 3] (c22) {Conversational interaction}}
child {node[level 3] (c23) {Textual entailment generation}}
child {node[level 3] (c24) {Information disguise}}
child {node[level 3] (c24) {Query suggestion}}};
%child {node[level 3, draw=none] (c24) {} edge from parent[draw=none]}};

\begin{scope}[every node/.style={level 4}]
%\node [below of = c21, xshift=2em] (c211) {Debiasing};
\node [below of = c21, xshift=2em] (c212) {Image recaptioning};
\node [below of = c212] (c213) {Positive Reframing};
\node [below of = c213] (c214) {Text localization};

\node [below of = c22, xshift=2em] (c221) {Argument repetition};
\node [below of = c221] (c222) {Question dodging};
\node [below of = c222] (c223) {Rogerian rhetoric application};
\node [below of = c223] (c224) {Utterance clarification};

%\node [below of = c23, xshift=2em] (c231) {Conclusion generation};

%\node [below of = c24, xshift=2em] (c241) {Information disguise};
%\node [below of = c241] (c242) {Query suggestion / expansion};
\end{scope}

% lines from each level 3 node to every one of its children
\foreach \value in {2,3,4}
\draw[<-] (c21.south west) |- (c21\value.west);

\foreach \value in {1,2,3,4}
\draw[<-] (c22.south west) |- (c22\value.west);

%\foreach \value in {1}
%\draw[<-] (c23.south west) |- (c23\value.west);

%\foreach \value in {1,2}
%\draw[<-] (c2.east) -- ++(2.4,0) -| ++(0,0) |- (c24\value.west);

\end{tikzpicture}
\egroup


